Medical Image Segmentation with SAM-generated Annotations

The field of medical image segmentation is hindered by the scarcity of large, publicly available annotated datasets. Not all datasets are made public for privacy reasons, and creating annotations for a large dataset is time-consuming and expensive, as it requires specialized expertise to accurately identify regions of interest (ROIs) within the images. To address these challenges, we evaluate the performance of the Segment Anything Model (SAM) as an annotation tool for medical data by using it to produce so-called "pseudo labels" on the Medical Segmentation Decathlon (MSD) computed tomography (CT) tasks. The pseudo labels are then used in place of ground truth labels to train a UNet model in a weakly-supervised manner. We experiment with different prompt types on SAM and find that the bounding box prompt is a simple yet effective method for generating pseudo labels. This method allows us to develop a weakly-supervised model that performs comparably to a fully supervised model.

==> sections/preliminaries.tex <==
\section{Preliminaries}\label{sec:pre}
This section introduces the main concepts used in our hybrid map compression, namely product quantization, map compression, and low-rank adaptation.

\boldparagraph{Product Quantization (PQ).}
PQ~\cite{jegou2010product} splits a high-dimensional vector space into smaller, more manageable subspaces that are then quantized independently.
%Each subspace is then quantized independently. 
A vector in the original high-dimensional space is transformed into the concatenation of the quantized codes from each subspace. Suppose we have a database $\{\bx\}$ of high-dimensional vectors $\bx \in \nR^D$, where $D$ is the dimensionality of the vector space.
%In Product Quantization, e
Each vector in the database is divided into $M$ sub-vectors, each of dimension $D' = D/M$, \ie $\bx=[\bx_1,\bx_2,...,\bx_M]$, where $\bx_m$ is the $m$-th sub-vector of $\bx$.
For each subspace $m$, a codebook $\mathbf{C}_m \in \mathbb{R}^{K \times D'}$ of $K$ centroids is trained on $\{\bx_m\}$ using K-Means~\cite{bishop2006pattern}.
This results in $M$ codebooks $\mathbf{C} = [\mathbf{C}_1...\mathbf{C}_m...\mathbf{C}_M]$. 
%
Each sub-vector $\bx_m$ is then quantized independently into the index $q_m$ of the centroid closest to in $\bx_m$ the codebook $\mathbf{C}_m$:
%
%Each sub-vector $\bx_m$ is then quantized independently into $q_m$ by mapping $\bx_m$ to the closest centroid in $\mathbf{C}_m$:
%. For the subspace, $m$, the quantization process can be represented as:
%
\begin{equation}
\label{eq:final-loss}
q_m = \argmin_{\bc \in C_m} \| \bx_m - \bc \|
\end{equation}
%
%\noindent The result of this quantization is the index $q_m$ of the closest centroid in the codebook $\mathbf{C}_m$. 
%
\noindent The tuple of indices $(q_1,...q_m,...q_M)$ from all $M$ subspaces forms the quantized representation of the original vector. The original vector can be approximated by concatenating the centroids corresponding to these indices.


\boldparagraph{Map Compression.}
We adopt the map compression of~\cite{mera2020efficient}, also used in~\cite{Yang_2022_CVPR}, to select 3D points that are both distinctive and spatially far away from each other to provide uniform coverage of the scene. 
%
%Map compression~\cite{mera2020efficient,Yang_2022_CVPR} is a popular technique for reducing the database memory by removing redundant 3D points from the map. The main idea is to select 3D points that are both distinctive and spatially far away from each other to provide uniform coverage of the scene.
This is done by solving the following optimization problem where $v$ represents a discrete probability distribution over the 3D points that has non-zero values on the selected points:
%
\begin{equation}
\begin{aligned}
  \min_{v} \hspace{2mm} v^T K v - \tau d^T v \\
  \textrm{s.t.} \sum_{i}^{m} v_i = 1, \ \ \  0 \leq v_i \leq \frac{1}{\alpha m};
\end{aligned}
\label{eq:map_compr}
\end{equation}
%
$\alpha \in  (0,1]$ is the compression ratio with lower $\alpha$ resulting in higher map compression.
$K$ is the distance matrix storing the Euclidean distance between all pairs of 3D points, and $d$ is a vector that defines the distinctiveness of a 3D point as the fraction of total images (cameras) observing that 3D point.

\boldparagraph{Low-Rank Adaptation.} LoRA~\cite{hu2021lora}
%has gained prominence as a way
allows
to fine-tune large models on specific tasks without the need to retrain the entire model, which can be computationally expensive and time-consuming.
To do so, it
%The main idea behind LoRA is to 
adapts only a small subset of the model's weights during the fine-tuning process. 
Instead of updating all the weights of a neural network, LoRA targets specific layers (\eg, linear layers) and introduces low-rank matrices that capture task-specific adaptations. Specifically, let us consider a weight matrix $W\in\nR^{d_\text{in}\times d_\text{out}}$ where $d_\text{in}$ and $d_\text{out}$ represent the input and output dimension, respectively. Instead of updating $W$ directly during fine-tuning, we keep $W$ fixed and introduce two matrices, $B\in\nR^{d_\text{in}\times r}$ and $A\in\nR^{r \times d_\text{out}}$, where $r$ is the rank which is much smaller than $d_\text{in}$ and $d_\text{out}$. The effective adaptation of the weight matrix $W$ is then computed as: $W^{\prime}=W + BA$.
%\begin{equation}
%    W^{\prime}=W + BA
%\end{equation}
\noindent During training, only low-rank matrices $A$ and $B$ are updated, and $W$ remains unchanged. 

%In~\cref{sec:results-lora} we show how to efficiently apply LoRA in the camera relocalization domain when the memory budget is limited.

%\subsection{Task Formulation}
%Full Pipeline from PQ to 3D map compression to training to localization (either here or earlier?)


